Motor State Prediction and Friction Compensation for Brushless DC Motor Drives Using Data-Driven Techniques

In order to provide robust, reliable, and accurate position and velocity control of motor drives, friction compensation has emerged as a key difficulty. Non-characterised friction could give rise to large position errors and vibrations which could be intensified by stick-slip motion and limit cycles. This paper presents an application of two data-driven nonlinear model identification techniques to discover the governing equations of motor dynamics that also characterise friction. Namely, the extraction of low-power data from time-delayed coordinates of motor velocity and sparse regression on nonlinear terms was applied to data acquired from a Brushless DC (BLDC) motor, to identify the underlying dynamics. The latter can be considered an extension of the conventional linear motor model commonly used in many model-based controllers. The identified nonlinear model was then contrasted with a nonlinear model that included the LuGre friction model and a linear model without friction. A nonlinear grey box model estimation method was used to calculate the optimum friction parameters for the LuGre model. The resulting nonlinear motor model with friction characteristics was then validated using a feedback friction compensation algorithm. The novel model showed more than 90% accuracy in predicting the motor states in all considered input excitation signals. In addition, the model-based friction compensation scheme showed a relative increase in performance when compared with a system without friction compensation.

==> Dump.tex <==
\begin{figure*}[!t]

\begin{equation}
\mathit{ 
\Theta (\bm{X},\bm{U})^T
= \begin{bmatrix}
  \bm{X} \\
\bm{\dot{X}}\\
\bm{Z}\\
\bm{I}\\
 tanh (a \bm{\dot{X}})  \\
 tanh (a \bm{Z})  \\
\bm{|\dot{X}|\dot{X}}\\
\bm{|\dot{X}|\dot{X^2}}\\
\bm{|Z|Z}\\
\bm{|Z|{Z^2}}\\
\bm{Z\dot{X}}\\
\bm{Z^2\dot{X}}\\
\bm{Z\dot{X}^2}\\
\bm{U} \\
\bm{ZU} \\
\bm{Z^2U} \\
\bm{ZU^2} \\
\end{bmatrix}
 \Xi = \begin{bmatrix}
0 &	0 & 0 &	0 \\
1.14 & -16.00 &	3.55\times10^{-3} &	-1.95 \\
0 & -4331.86 &	-57.80 & 118.95 \\
0 &	-53.76 & 0 & -29.87 \\
0 &	-8.23 &	0.51 &	-0.66 \\
0 & 0 & 0.17 & -0.33 \\
0 & -0.03 & -8.76\times10^{-5} & 7.70\times10^{-4} \\
0 & -6.61\times10^{-6} & 0 &	0 \\
0 & 50296.02 & 0 & 0 \\
0 & 24866.62 & 476.10 & 997.65 \\
0 & -12.40 & 0 & 0 \\
0 & 188.93 & 0 & -53.11 \\
0 & -0.18 & 0 & 8.75\times10^{-3} \\
0 & 244.79 & 0 & 25.07 \\
0 & 97.73 & 0 & 0 \\
0 & 0 & 0 & 701.42 \\
0 & -23.37 & 0 & 0 \\
\end{bmatrix}}
\label{eq:42}
%\end{equation}
%\normalsize
%\end{align*}
\end{equation}
%\end{strip}
\end{figure*}
